Exciting Nucleons in Compton Scattering and Hydrogen-Like Atoms

This PhD thesis is devoted to the low-energy structure of the nucleon (proton and neutron) as seen through electromagnetic probes, e.g., electron and Compton scattering. The research presented here is based primarily on dispersion theory and chiral effective-field theory. The main motivation is the recent proton radius puzzle, which is the discrepancy between the classic proton charge radius determinations (based on electron-proton scattering and normal hydrogen spectroscopy) and the highly precise extraction based on first muonic-hydrogen experiments by the CREMA Collaboration. The precision of muonic-hydrogen experiments is presently limited by the knowledge of proton structure effects beyond the charge radius. A major part of this thesis is devoted to calculating these effects using everything we know about the nucleon electromagnetic structure from both theory and experiment. The thesis consists of eight chapters. The first and last are, respectively, the introduction and conclusion. The remainder of this thesis can roughly be divided into the following three topics: finite-size effects in hydrogen-like atoms, real and virtual Compton scattering, and two-photon-exchange effects.

==> Sec2Introduction.tex <==
\chapter{Introduction to Compton Scattering and Hydrogen Theory}
\section{Notations and Conventions}

Here we list the notations and conventions used throughout this thesis. Unless specified, all calculations are presented in natural units, $\hbar=c=1$, and we use the following notations for the well-established parameters, along with their 
Particle Data Group (PDG) values \cite{Agashe:2014kda}:
\begin{itemize}
\item[$\al$] the fine-structure constant, $\al = e^2/4\pi=1/137.035\,999\,074(44)$.
\item[$\hbar c$] conversion constant, $\hbar c=197.326 \,9718(44) \, \mathrm{MeV}\,\mathrm{fm}$.
\item[$m$]   lepton mass, $\{m_e, m_\mu \} \simeq \{0.510\,998\,928(11), 105.658\,3715(37)\}\,\mathrm{MeV}$.
\item[$m_\pi$] pion mass, $\{m_{\pi^0}, m_{\pi^\pm}\}\simeq \{134.9766(6), 139.570\,18(35)\}\,\mathrm{MeV}$.
\item[$M$]   nucleon mass, $\{M_p, M_n\} \simeq \{938.272\,046(21), 939.565\,379(21)\}\,\mathrm{MeV}$.
\item[$\varkappa $]   nucleon anomalous magnetic moment, 
$(\varkappa_p, \varkappa_n) \simeq (1.7929,\, -1.9130 )$.
\end{itemize}
Furthermore, we introduce the Minkowski metric:
\begin{equation}g=
\left(
\begin{array}{cccc}
 1 & 0 & 0 & 0 \\
 0 & -1 & 0 & 0 \\
 0 & 0 & -1 & 0 \\
 0 & 0 & 0 & -1
\end{array}
\right),
\end{equation}
to define the four-vector scalar product:
\begin{equation}
a \cdot b= g_{\rho \sigma} \,a^\rho b^\sigma = a_\sigma b^\sigma =  a_0b_0 - \boldsymbol {a}\cdot \boldsymbol{b},
\end{equation} 
and utilize the Einstein summation convention to sum over repeated indices.
\section{Nucleon Form Factors}
\subsection{Moments of Charge and Magnetization Distributions}
\section{Theory of Compton Scattering}
\subsection{Polarizabilities in Compton Scattering}
\subsection{Doubly-Virtual Compton Scattering}
\subsubsection{Low-Energy Expansion of Compton Amplitudes}
\subsubsection{Sum Rules for Compton Amplitudes}
\section{Proton Structure in Hydrogen}
\subsection{The Hydrogen Spectrum}
\subsection{Finite-Size Effects: Charge Radius and Beyond}
\subsection{Structure Effects Through Two-Photon Exchange}
\subsubsection{Two-Photon Exchange in Terms of Compton Amplitudes}
\subsubsection{Master Formulae in Terms of Proton Structure Functions}
\subsubsection{Seperating Nucleon-Pole and Inelastic Contributions}
\paragraph*{Nucleon-Pole Contribution}
\paragraph*{Inelastic Contribution}
\paragraph*{Ambiguity of the Nucleon-Pole Contribution}
\subsubsection{Rearrangement into Born and Polarizability Contributions}
\subsubsection{Two-Photon Exchange in the Lamb Shift}
\paragraph*{Born Contribution}
\paragraph*{Polarizability Contribution}
\subsubsection{Two-Photon Exchange in the Hyperfine Splitting}
\paragraph*{Born Contribution}
\paragraph*{Polarizability Contribution}
\begin{subappendices}
\section{Hyperspherical Coordinates and Wick Rotation}
\end{subappendices}


